Ask & Explore: Grounded Question Answering for Curiosity-Driven Exploration

In many real-world scenarios where extrinsic rewards to the agent are extremely sparse, curiosity has emerged as a useful concept providing intrinsic rewards that enable the agent to explore its environment and acquire information to achieve its goals. Despite their strong performance on many sparse-reward tasks, existing curiosity approaches rely on an overly holistic view of state transitions, and do not allow for a structured understanding of specific aspects of the environment. In this paper, we formulate curiosity based on grounded question answering by encouraging the agent to ask questions about the environment and be curious when the answers to these questions change. We show that natural language questions encourage the agent to uncover specific knowledge about their environment such as the physical properties of objects as well as their spatial relationships with other objects, which serve as valuable curiosity rewards to solve sparse-reward tasks more efficiently.

==> reviews.tex <==
Reviewer #1
Questions
1. [Summary] Please briefly summarize the paper in 1-2 sentences.
This paper presents a linguistic curiosity method for encouraging exploration in RL. The method involves training a visual-question-answering (VQA) model to answer referential questions like “are there any purple balls next to the red ball?”. Then the agent is provided an intrinsic reward in states where the VQA model changes answers. Experiments show the proposed approach outperforms other curiosity methods in the CLEVR-Robot environment.
2. [Rating] Please provide an "overall score" for this submission.
Accept
3. [Justification of Rating] Please briefly justify your rating.
Overall, this paper presents a very promising approach for curiosity driven exploration. Not all states are interesting, so using language to semantically guide an agent towards meaningful exploration could be valuable for efficient RL. The preliminary results are also promising, and with a few more experiments across multiple domains, this work could be potentially submitted to an ML venue (like ICLR or NeurIPS).

Detailed Comments:
Section 3, Para 2: The approach makes one big assumption that the agent has access to this set of Question Q1, Q2 … QN. It might be easy to define these questions in CLEVR-Robot since the dataset was specifically designed for reference resolution. Defining such questions in other domains (like Mujoco tasks or other robot control problems) can be non-trivial or impossible. At some point, constructing these questions might also become a form domain-specific feature engineering. One can imagine building a set of ‘symbolic’ predicates like “right_of(red, blue)” etc. and training a simple classifier to classify these unary/binary features. Would that be a good alternative for language-based VQA models?

Section 4.1, Para 1: In “There is a green sphere; are there any rubber cyan balls in front of it”, what is the goal here? – this seems like a question, but the goal is a physical action?

Section 4.2, Para 4: What exactly was this n=1 single question that worked so well?

Figure 3b: Why just n=1 in the sparse setting? Why not n=2 and n=1280 like with the dense setting?

Section 4: The empirical results could be greatly strengthened if this approach works beyond CLEVR-Robot. Are there other domains where linguistic curiosity could be helpful? Since VQA models are just trained on Image-Question pairs, can you train one VQA model across domains, and show that linguistic curiosity can be transferred across domains since referential semantics are universal?
Reviewer #3
Questions
1. [Summary] Please briefly summarize the paper in 1-2 sentences.
The paper proposes a methodology to generate intrinsic rewards to encourage agent exploration. Particularly, the paper investigates interactive tasks in the CLEVR-Robot Environment. The key hypothesis being investigated -- if exploration should be encouraged for certain states where the agent’s answer (to randomly sampled questions) changes. Particularly, it can be seen as an alternative take at popular exploration methods. For example, it could be seen as a count-based exploration that counts 'flipped-answers' instead of hashed state representations. Or, alternatively, it could be seen as an environment dynamic model with the twist of state features (Pathak et al. 2017) being replaced with answer distributions. The authors present results across two tasks with varying densities of supervision. Some results support the hypothesis (sparse reward task) while others indicate that the effect isn’t linear with the complexity of questions or number of questions.
2. [Rating] Please provide an "overall score" for this submission.
Reject
3. [Justification of Rating] Please briefly justify your rating.
A fair comparison with baselines:
From Section 3, a “labeling function of the CLEVR-Robot environment” or a “VQA model” is used for results in the main paper and Appendix D.2, respectively. After reading through both the main paper and the appendix, it isn't clear to the reviewer how $Q_k(s_t)$ is obtained. Regardless, it seems that the answer generation module isn’t trained with the model. Hence, it uses additional (labeled?) information that the three baselines don’t. Equipping the three baselines with as many QA tuples as the AnE method has access to, would be a fair comparison.

Generating answer distribution $Q_k(s_t)$ isn’t self-supervised:
Importantly, by definition, the calculation of 'intrinsic' rewards should be self-supervised. Accessing the labeling function or using QA tuples to train VQA models (like via Johnson et al.) cannot be part of a self-supervised 'intrinsic' reward formulation.

The claims of “asking questions” and “grounded language understanding” aren’t substantiated in experiments:
After reading through the appendix, particularly, the detailed algorithm 1, the reviewer finds the experiments to fall short of the claims of the paper. Particularly, the paper mentions the proposed approach encourages the agent to “ask questions” (abstract, introduction, figure 1, and conclusion) while the implementation shows that the questions are randomly sampled from a set of questions initialized ($q \sim S$). Further, the authors haven’t explained how $S$ is generated in the first place.
Similarly, the paper doesn’t delve into effectively evaluating "grounding" in any of the experiments. The fact that the questions sampled ask about spatial relationships doesn’t imply the AnE agent can ground language, vision, or actions. Correlations across language, vision, and actions must be studied, in some capacity, to draw such a bold (and indeed, impactful) inference.

Technical rigor:
(a) The notation of $Q_k$ is overloaded. It denotes the questions as well as an operator over the states, which is confusing.
(b) Sec. 4.1 details two tasks where a reward of 1 or 10 is available at the successful completion of the task. The "dense" and "sparse" nature of the reward structure for the MDPs isn't clear to the reviewer.


Suggestions:
(a) QA-based curiosity is indeed an exciting direction that the authors investigate. However, the reviewer is unsure of the formulation of this direction. Why should a change in the agent’s answer distribution from $s_t$ to $s_{t+1}$ indicate ‘curiosity’. For example, types and number of unique question generations or a non-peaky to peaky shift in the answer distribution (unsure to sure transition in the agent’s world model) seem like more direct realizations of the author’s goal to study QA-based curiosity in interactive agents.
(b) Mathematically grounded ‘distance’ between $Q_k(s_t)$ and $Q_k(s_{t+1})$ such as KL divergence, Jensen-Shannon divergence, or the total variation distance could be considered (in addition to the current sample and count).
(c) Additional visual curiosity references:
-- Scialom, Thomas, and Jacopo Staiano. "Ask to learn: A study on curiosity-driven question generation." arXiv preprint arXiv:1911.03350 (2019).
-- Yang, Jianwei, et al. "Visual Curiosity: Learning to Ask Questions to Learn Visual Recognition." Conference on Robot Learning. PMLR, 2018.

Kindly note the points summarized in this “suggestions” paragraph had no impact on the reviewer’s rating. It was objectively based on the experiments and the hypothesis the authors wish to investigate.
